Unique Parallel Decomposition for the Pi-calculus

A (fragment of a) process algebra satisfies unique parallel decomposition if the definable behaviours admit a unique decomposition into indecomposable parallel components. In this paper we prove that finite processes of the pi-calculus, i.e. processes that perform no infinite executions, satisfy this property modulo strong bisimilarity and weak bisimilarity. Our results are obtained by an application of a general technique for establishing unique parallel decomposition using decomposition orders.

==> eptcsdata.tex <==
\providecommand{\firstpage}{45}
\providecommand{\publicationstatus}{D. Gebler and K. Peters (Eds.): Combined Workshop on Expressiveness in\\
Concurrency and Structural Operational Semantics (EXPRESS/SOS 2016).\\
EPTCS 222, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.222.4}{10.4204/EPTCS.222.4}}

